Evaluating Policy Implications on the Restrictiveness of Flow-based Market Coupling with High Shares of Intermittent Generation: A Case Study for Central Western Europe

The current stage in the evolution of the European internal energy market for electricity is defined by the transformation towards a renewable energy system. The Clean Energy Package aims to ensure that methods for capacity allocation and congestion management, that are at the center of the European internal market for electricity, align with this transformation. Flow-based market coupling, the preferred method for capacity allocation, is first and foremost a formal process to allocate exchange capacities to the markets. However, the process also allows for many considerations of the involved parties that impact the resulting capacities. As part of the Clear Energy Package, the regulatory body enacted their ambition to increase exchange capacities by enforcing transmission system operators to allocate a minimum margin of physical line capacity with the goal of providing a higher level of competition and better integration of renewable energy sources. This study investigates this and other policy relevant consideration of flow-based market coupling. The model results quantify the trade-off between permissive capacity allocation and increased congestion management. For high shares of intermittent renewable generation, less constrained exchange capacities are favorable, however also highlight the importance of the markets ability to integrate high shares of intermittent generation. apacities are favourable, however also highlight the importance of the markets ability to integrate high shares of intermittent generation.

==> trunk.tex <==
\begin{table}[h]
\centering
\caption{Average marginal price and costs differences between CWE bidding zones in terms of target year and minRAM configuration}\label{tbl:price}
\begin{tabular}{@{}llllllllll@{}} \toprule
                      &             & \multicolumn{8}{c}{minRAM configuration}                                                                                                             \\ \cmidrule(l){3-10} 
                      &             & \multicolumn{2}{c}{20\%} & \multicolumn{2}{c}{40\%} & \multicolumn{2}{c}{70\%} & \multicolumn{2}{c}{70\% (only CB)} \\ \midrule
                      &             & $\Delta \lambda$  & $\sigma$       & $\Delta \lambda$            & $\sigma$       & $\Delta \lambda$            & $\sigma$       & $\Delta \lambda$                 & $\sigma$         \\
\multirow{2}{*}{2020} & D-1         & 24.41 & 0.94 & 22.4 & 0.95 & 21.23 & 0.91 & 17.06 & 0.91 \\ 
                      & D-0         & 15.87 & 1.12 & 25.6 & 1.08 & 30.56 & 1.02 & 35.65 & 0.95 \\ \midrule
\multirow{2}{*}{2030} & D-1         & 31.73 & 1.33 & 24.62 & 1.14 & 22.49 & 1.15 & 19.46 & 1.17 \\ 
                      & D-0         & 11.54 & 0.99 & 11.64 & 1.01 & 11.73 & 1.02 & 12.61 & 1.02 \\ \bottomrule
\end{tabular}
\end{table}

% Table generated by Excel2LaTeX from sheet 'price_table_final'
\begin{table}[htbp]
  \centering
  \caption{Average price $\lambda$ and price differences $\Delta \lambda$ in- and between CWE bidding zones in terms of year and minRAM configuration}\label{tbl:price}
    \begin{tabular}{clllllllll}
    \toprule
          &       & \multicolumn{2}{c}{20\%} & \multicolumn{2}{c}{40\%} & \multicolumn{2}{c}{70\%} & \multicolumn{2}{c}{70\% (only CB)} \\
\cmidrule{3-10}          &       & \multicolumn{1}{l}{$\lambda$} & \multicolumn{1}{l}{$\Delta \lambda$} & \multicolumn{1}{l}{$\lambda$} & \multicolumn{1}{l}{$\Delta \lambda$} & \multicolumn{1}{l}{$\lambda$} & \multicolumn{1}{l}{$\Delta \lambda$} & \multicolumn{1}{l}{$\lambda$} & \multicolumn{1}{l}{$\Delta \lambda$} \\
    \midrule
    \multirow{2}[1]{*}{2020} & market & 50.02 & 24.41 & 44.68 & 22.4  & 41.61 & 21.23 & 39.08 & 17.06 \\
          & redispatch & 55.81 & 15.87 & 64.84 & 25.6  & 69.12 & 30.56 & 72.73 & 35.65 \\ \midrule
    \multirow{2}[1]{*}{2030} & market & 43.47 & 31.73 & 42.02 & 24.62 & 41.3  & 22.49 & 37.58 & 19.46 \\
          & redispatch & 58.76 & 11.54 & 59.88 & 11.64 & 60.89 & 11.73 & 62.92 & 12.61 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%
